Scaling New Frontiers: Insights into Large Recommendation Models

Recommendation systems are essential for filtering data and retrieving relevant information across various applications. Recent advancements have seen these systems incorporate increasingly large embedding tables, scaling up to tens of terabytes for industrial use. However, the expansion of network parameters in traditional recommendation models has plateaued at tens of millions, limiting further benefits from increased embedding parameters. Inspired by the success of large language models (LLMs), a new approach has emerged that scales network parameters using innovative structures, enabling continued performance improvements. A significant development in this area is Meta's generative recommendation model HSTU, which illustrates the scaling laws of recommendation systems by expanding parameters to thousands of billions. This new paradigm has achieved substantial performance gains in online experiments. In this paper, we aim to enhance the understanding of scaling laws by conducting comprehensive evaluations of large recommendation models. Firstly, we investigate the scaling laws across different backbone architectures of the large recommendation models. Secondly, we conduct comprehensive ablation studies to explore the origins of these scaling laws. We then further assess the performance of HSTU, as the representative of large recommendation models, on complex user behavior modeling tasks to evaluate its applicability. Notably, we also analyze its effectiveness in ranking tasks for the first time. Finally, we offer insights into future directions for large recommendation models. Supplementary materials for our research are available on GitHub at https://github.com/USTC-StarTeam/Large-Recommendation-Models.

==> Tables/dataset.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{@{}lcccc@{}}
    \toprule
    \textbf{Datasets} & \textbf{\#Users} & \textbf{\#Items} & \textbf{\#Pos. Inters.} & \textbf{\#Neg. Inters.} \\
    \midrule
    ML-1M   & 6,040   & 3,706   & 575,281   & 424,928   \\
    ML-20M  & 138,493 & 26,744  & 9,995,410 & 10,004,853 \\
    AMZ-Books   & 694,897 & 686,623 & 8,150,484 & 1,902,602 \\
    \bottomrule
    \end{tabular}
    \caption{Statistics of different datasets}
    \label{tab:dataset_statistics}
\end{table}


==> Tables/huawei_music_offline.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{c >{\dope}p{1.4cm} >{\dope}p{1.4cm} >{\dope}p{1.4cm} >{\dope}p{1.4cm} >{\dope}p{1.4cm} @{}}
        \toprule
        \textbf{Model} & \textbf{HR@10} & \textbf{HR@50} & \textbf{NDCG@10} & \textbf{NDCG@50} & \textbf{MRR} \\ 
        \midrule
        SASRec & 0.1625 & 0.2252 & 0.2949 & 0.5752 & 0.1389 \\
        Llama & 0.2216 & 0.2779 & 0.3714 & 0.6228 & 0.1907 \\
        HSTU & 0.2291 & 0.2852 & 0.3823 & 0.6328 & 0.1970 \\
        FuXi-$\alpha$ & 0.2480 & 0.3023 & 0.4061 & 0.6484 & 0.2138 \\
        \bottomrule
    \end{tabular}
    \caption{Hello World.}
    \label{tab:huawei_music_offline}
    \vspace{-5mm}
\end{table*}

==> Tables/huawei_music_online.tex <==
\begin{CJK*}{UTF8}{gbsn}
\begin{table*}[ht]
    \centering
    \begin{tabular}{c >{\dope}p{3.0cm} >{\dope}p{3.0cm} >{\dope}p{3.0cm} @{}}
        \toprule
        \textbf{Date} & \textbf{歌曲播放次数} & \textbf{歌曲播放设备数} & \textbf{歌曲播放时长\hspace{0.075cm}(秒)} \\ 
        \midrule
        20241111 & 0.80\% & 1.10\% & 0.27\% \\
        20241112 & 1.35\% & 1.21\% & 1.39\% \\
        20241113 & 0.08\% & 0.45\% & -0.58\% \\
        20241114 & 2.18\% & 1.74\% & 2.14\% \\
        20241115 & 1.41\% & 1.60\% & 0.79\% \\
        20241116 & 1.16\% & 0.99\% & 0.76\% \\
        20241117 & 0.53\% & -0.17\% & 0.01\% \\
        \bottomrule
    \end{tabular}
    \caption{Hello World.}
    \label{tab:huawei_music_online}
    \vspace{-5mm}
\end{table*}
\end{CJK*}

==> Tables/huawei_music_online_radar.tex <==
\begin{CJK*}{UTF8}{gbsn}
\begin{table*}[ht]
    \centering
    \begin{tabular}{c >{\dope}p{3.0cm} >{\dope}p{3.0cm} >{\dope}p{3.0cm} @{}}
        \toprule
        \textbf{Date} & \textbf{歌曲播放次数} & \textbf{歌曲播放设备数} & \textbf{歌曲播放时长\hspace{0.075cm}(秒)} \\ 
        \midrule
        20241104 & 0.88\% & -0.09\% & 4.91\% \\
        20241105 & 0.15\% & 0.85\% & 2.37\% \\
        20241106 & -0.45\% & -0.29\% & 2.51\% \\
        20241107 & 3.38\% & 1.92\% & 6.25\% \\
        20241108 & 0.84\% & 0.01\% & 4.58\% \\
        20241109 & 0.54\% & 0.01\% & 3.89\% \\
        20241110 & 3.65\% & 0.06\% & 7.52\% \\
        \bottomrule
    \end{tabular}
    \caption{Hello World.}
    \label{tab:huawei_music_online_radar}
    \vspace{-5mm}
\end{table*}
\end{CJK*}

==> Tables/ltable.tex <==
\begin{table}[t]
\centering
\small
    \begin{tabular}{@{} c c >{\dope}p{1.2cm} >{\dope}p{1.2cm} >{\dope}p{1.2cm} >{\dope}p{1.2cm} @{}}
    \toprule
    \textbf{Length} & \textbf{\# Blocks} & \textbf{NDCG@10} &\textbf{NDCG@50} & \textbf{HR@10} &\textbf{MRR}\\
    \midrule
    \multirow{4}{*}{600} & 4     &    0.3790 & 0.4308 & 0.5898  &0.3273 \\ 
    & 8    &  0.3691 & 0.4176 &0.5967  & 0.3114 \\ 
    & 12   &  0.3354 &0.3880 & 0.5703  & 0.2765 \\ 
    & 16   & 0.2640 & 0.3234 & 0.4941  &0.2102 \\ 
    \midrule
    \multirow{4}{*}{400} & 4  & 0.3319 & 0.3903 & 0.5291 & 0.2832 \\ 
    & 8    &       0.3362 & 0.3981 & 0.5332  & 0.2912 \\ 
    & 12    &      0.2917 & 0.3524 & 0.5068  & 0.2420 \\ 
    & 16    &       0.2634 & 0.3317 & 0.4648 & 0.2198 \\ 
    \bottomrule
    \end{tabular}
\caption{Performance of the HSTU model on KuaiRand-27k.}
\vspace{-8mm}
\label{Kuairand-27k}
\end{table}


==> Tables/ranking_withoutloss.tex <==
\begin{table*}[h!]
    \centering
    \begin{tabular}{@{}ccccc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\# Blocks}} & \multicolumn{3}{c}{\textbf{AUC}} \\
    ~ & ~ & \textbf{ML-1M} & \textbf{ML-20M} & \textbf{AMZ-Books} \\
    \midrule
    \multirow{1}{*}{DIN}
    & - & 0.7238 & 0.7245 & 0.7115 \\
    \midrule
    \multirow{6}{*}{HSTU} 
    & 2  & 0.7559 & 0.7813 & 0.7257 \\
    & 4  & 0.7530 & 0.7920 & 0.7386 \\
    & 8  & 0.7591 & 0.7960 & 0.7062 \\
    & 16 & 0.7943 & 0.7879 & 0.7252 \\
    & 24 & 0.7943 & 0.7992 & 0.7450 \\
    & 32 & 0.7947 & 0.7914 & 0.7606 \\
    \midrule
    \multirow{6}{*}{\hspace{0.5cm}Llama\hspace{0.5cm}} 
    & 2  & 0.7922 & 0.7568 & 0.7181 \\
    & 4  & 0.7923 & 0.7595 & 0.7585 \\
    & 8  & 0.7939 & 0.7375 & 0.7449 \\
    & 16 & 0.7915 & 0.6390 & 0.7469 \\
    & 24 & 0.7883 & 0.5777 & 0.7517 \\
    & 32 & 0.7923 & 0.7107 & 0.7491 \\
    \bottomrule
    \end{tabular}
    \caption{Performance of HSTU and Llama for the ranking task on 3 different datasets (ML-1M, ML-20M, and AMZ-Books). Note that a higher value indicates a better performance for the AUC metric.}
    \vspace{-7mm}
    \label{tab:ranking}
\end{table*}


==> Tables/ztable.tex <==
\begin{table}[h!]
\centering  
\begin{tabular}{@{} c >{\dope}p{1.5cm} >{\dope}p{1.5cm} @{}}
    \toprule
    \textbf{Model} & \textbf{HR@50} & \textbf{NDCG@50} \\
    \midrule
    Llama & 0.5489 & 0.2238 \\
    {\hspace{0.5cm}Llama w/ b\hspace{0.5cm}} & 0.5446 & 0.2205 \\
    \midrule
    HSTU & 0.5571 & 0.2297 \\
    {\hspace{0.5cm}HSTU w/ b\hspace{0.5cm}} & 0.5590 & 0.2333 \\
    \bottomrule
\end{tabular}
\caption{Performance of the Llama and HSTU models on the Huawei Music dataset. The ``w/ b'' model variant indicates explicit behavior modeling.}
\label{tab:performance_metrics}
\end{table}
